Understanding process-structure-property relation for elastoplastic behavior of polymer nanocomposites with agglomeration anomalies and gradient interphase percolation

For polymer nanocomposites, disordered microstructural nature makes processing control and tailoring properties to desired values a challenge. Understanding process-structure-property relation can provide guidelines for process and constituents design. Our work explores nuances of PSP relation for polymer nanocomposites with attractive pairing between particles and polymer bulk. In the absence of any nano or micro-scale local property measurement, we develop a material model that can represent decay for small strain elastoplastic properties in interfacial regions and simulate representative or statistical volume element behavior. This interfacial model is further combined with a microstructural design of experiments for agglomerated nanocomposite systems. Agglomerations are particle aggregations that are microstructural defects resulting from lack of processing control. Twin screw extrusion process can reduce extent of aggregation in hot pressed samples via erosion or rupture depending on screw rpms and toque. We connect this process-structure relation to structure-property relation that emerges from our study. We discover that balancing between local stress concentration zone and interfacial property decay governs how fast yield stress can improve if we break down agglomeration via erosion. Rupture is relatively less effective in helping improve nanocomposite yield strength. Additionally, we allude to yield initiation and progression in these multiphase materials. We have come up with a field quantity called local yield resistance that indicates balance stress concentration zones and interfacial effects. Yield resistance map from linear regime acts as a predictor of local yielding process and can be a useful tool for interface design for plastic deformation behavior.

==> prajakta.tex <==
\section{Inelastic Interphase material properties}\label{app.B}
\subsection{Interphase percolation}
Here, we have extended the 2D interphase approach, explained in section 1.2, to create a 3D interphase from a two-phase(particle and matrix) 3D microstructure image. In addition to that, we have also developed a capability to treat agglomeration anomalies as a single aggregate for a single body gradient and compounding interaction with other isolated particles or agglomerations. 

Interphase for the nanocomposites shows a complex mechanism of the single and multibody compounding effect (see Supplementary information). A 2D gradient interphase model, as shown in Figure \ref{fig:interphase}, consists of particles, matrix, and gradient interphase region. We extended the 2D model by taking the 3D reconstructed microstructures (see Section 2.3) and adding the interphase layer around the isolated and agglomerated particles. Next, we create finite layers for material property assignments for the interphase region for the ROM simulations. These layers can be used to assign a variety of macroscopic material properties like thermal, elastic, inelastic, viscoelastic, and glass transition (see Figure \ref{fig:inter_prop}).
%Set of parameters $\alpha^\prime,\beta^\prime,\eta^\prime,\zeta^\prime$  used for multiple properties can be identical or independent based on available experimental measurement or theoretical understanding of underlying processes and mechanisms of the macroscopic property. 
%Figure XX shows a flow schematic of this process. 


In this work, we use glass transition temperature as a basis for deriving an inelastic property profile. We assume that underlying interfacial molecular mechanisms that produce local property changes in elastic stiffness are very much the same that alter the local glass transition. Hence, we use a set of parameters that have been inferred from elastic property profile measurement from AFM data of model composites \cite{LI2019100277}  for describing local glass transition temperature variation. Further, for ease of computation at the micro and mesoscale, the gradient property description has been simplified and represented using a uniform interphase description.

\subsection{Inelastic Interphase material properties}\label{app.B}
In the absence of local property data beyond the linear material regime for polymer nanocomposites, we utilize data from local elastic modulus measurement to infer the effect of interfacial interactions on molecular mobility and glass transition temperature and ultimately to propose a material model for inelastic (yield) properties of the interphase. There have been multiple experimental studies that have tried to quantify the effect of operating temperatures on the macroscopic mechanical behavior of neat polymers. They all point to the fact that the stress-strain behavior of macroscopic polymers under mechanical loading greatly depends on operating temperatures relative to their glass transition temperatures.   It has been specifically observed for amorphous polymers that modulus in the linear regime,  yield stress decreases, and initial hardening in the nonlinear regime begins to diminish as operating temperatures approach glass transition temperature. A cooperative model of yield process rooted in molecular theories has been proposed and refined through the cumulative work of multiple researchers over the years. This model states that the yield process involves the cooperative motion of chain segments governed by glass transition temperatures, $T_g$, and molecular mobility. At temperatures below $T_g$, the polymer chains do not have enough thermal energy and mobility to undergo cooperative movements and act stiffer, recording higher yield stress values but exhibiting brittle failure. On the other hand, at temperatures approaching or above $T_g$, thermal energy, and mobility can afford cooperative chain movements and record lower yield values along with more ductile failure and high toughness.
We use this understanding to propose a temperature shift model that can be used to derive interphase material properties based on polymer bulk property data. Here we use yield stress as a sample property to explain the model. As explained by the cooperative model, the yield strength drops as the use temperature approaches the polymer glass transition temperature. If we assume attractive interfacial interactions, the polymer in the interphase region exhibits reduced chain mobility and overall reduction and delay in cooperative chain movements. This change would correspond to an increase in the extent of the linear regime and push the yield stress value upwards. We assume that the amount by which polymer yield stress can increase in the interphase region is related to the local change in $T_g$ of the interfacial region polymer. Thus, the yield-temperature curve of interphase can be obtained by shifting the same for neat polymer by amount and direction of change in $T_g$ (see Figure \ref{fig:prop}).

Conceptually, a similar approach can be adopted to derive other key properties in inelastic or non-linear deformation regimes. For example, strain hardening or softening beyond yield measured tangent modulus. Such extrapolations will require a detailed understanding of underlying molecular processes and how they are being altered within the interphase region by interfacial interactions. This is a topic of extensive and independent research that can combine molecular mobility theories and constitutive modeling at the macroscopic level. For the current purpose of broader and across-the-scale method development, we simplify our approach to selecting from available macroscopic property data that comes from extensive experimental research work about the effect of temperature on the stress-strain relation of polymer materials.

The development of interphase property gradients has a complex mechanism which consists of a “single body” effect for the interphase around a single isolated particle, and a “multibody compounding” effect for the property gradients between sufficiently close particles. [Li ref] (See supplemental information.) A 2D gradient interphase model, as illustrated in Figure \ref{MicroFramework}f-g, consists of particles, matrix, and gradient interphase region. We extended the 2D model by taking the 3D reconstructed microstructures (Section 2.3) and adding the graded interphase layer around the isolated and agglomerated particles (Figure \ref{MicroFramework}l).

For the elastic interphase properties, we use guidance from AFM experiments [refs 29, 30, add others] which have carefully examined model and in situ interphases and provided data on the extent and magnitude for the gradient elastic properties of a glassy polymer in the interphase regime in both the single body and multibody effect regimes. We use the magnitude and functional form determined from these experiments to create the model framework for simulations of the elastic property gradients. The graded interphase is most generally represented by a finite number of discrete layers of changing properties as illustrated in Figures 5 and 6.  However, to simplify the multiscale ROM simulations in the later design studies, we the interphase is represented with a single layer of uniform properties. This approach allows for the impact of the interphase properties to be included while facilitating efficient simulation pathways for the design and optimization process. 
Due to the lack of direct measurement of local inelastic properties in the interphase regime, in this work we use glass transition temperature ($T_g$) as a basis to derive a reasonable estimation of the inelastic property profile. We assume that underlying interfacial molecular mechanisms that produce local property changes in both $T_g$ and elastic stiffness impact yield stress in a similar fashion and use this assumption to develop a material model for the inelastic (yield) properties of interphase. Based on experimental studies, it is clear that the macroscopic stress-strain behavior of polymers greatly depends on operating temperatures relative to their $T_g$. It has been specifically observed for amorphous polymers that yield stress decreases, and initial hardening in the nonlinear regime begins to diminish as operating temperatures approach the $T_g$ from below [refs]. This observation is due to the dependence of the yield process on cooperative motion of chain segments governed by the $T_g$ and molecular mobility. At temperatures below $T_g$, the lower thermal energy and mobility of polymer chains inhibit cooperative movements, resulting in increased yield stress values and more brittle failure processes. We use this understanding to propose a temperature shift model that can be used to derive inelastic interphase properties based on bulk polymer property data. 
As explained by the cooperative model, the yield strength increases as the use temperature decreases from the polymer $T_g$. If we assume attractive interfacial interactions, the polymer in the interphase region exhibits reduced chain mobility and overall reduction and delay in cooperative chain movements. This change corresponds to an effective increase in the local $T_g$, as has been consistently observed [torkelson and other refs]. Consequently, this effective increase in the local $T_g$, has the effect of increasing the extent of the linear regime and pushing the yield stress value higher. We use this understanding to propose a temperature shift model that can be used to derive inelastic interphase properties based on bulk polymer property data. 
